Probabilistic 3D Multi-Modal, Multi-Object Tracking for Autonomous Driving

Multi-object tracking is an important ability for an autonomous vehicle to safely navigate a traffic scene. Current state-of-the-art follows the tracking-by-detection paradigm where existing tracks are associated with detected objects through some distance metric. The key challenges to increase tracking accuracy lie in data association and track life cycle management. We propose a probabilistic, multi-modal, multi-object tracking system consisting of different trainable modules to provide robust and data-driven tracking results. First, we learn how to fuse features from 2D images and 3D LiDAR point clouds to capture the appearance and geometric information of an object. Second, we propose to learn a metric that combines the Mahalanobis and feature distances when comparing a track and a new detection in data association. And third, we propose to learn when to initialize a track from an unmatched object detection. Through extensive quantitative and qualitative results, we show that when using the same object detectors our method outperforms state-of-the-art approaches on the NuScenes and KITTI datasets.

==> figures/flowchart_old.tex <==
\begin{figure*}[t!]
    \centering
    %\includegraphics[width=1.0\linewidth]{img_new/architecture_zoom_in_v1.png}
    \includegraphics[width=1.0\linewidth]{img_new/architecture_2020_1031_0749.pdf}
    
    %\caption{Algorithm Flowchart. Our proposed multi-object tracking algorithm is built using Kalman filters. We adapt three learning modules to conduct 2D/3D feature fusion, data association measurement and new track initialization detection. We ignore ReLU layers in the network structures following every convolutional and linear regression layers for illustration simplicity.}
    \caption{Algorithm Flowchart. The left part shows the hight level overview of our proposed architecture, and the right part illustrates the details of each neural network module. At frame $t$, We use a 3D object detector and extract the LiDAR and image features for each detected object. These features are fused by the \textit{Feature Fusion Module}. The fused features of detections from time $t$ and tracks from time $t-1$ are used in the \textit{Trainable Distance Combination Module} to learn the combination of the deep feature distance and the Mahalanobis distance. We apply a greedy match algorithm on the combined distance for data association. Matched pairs are further processed by the Kalman Filter to refine the final object states. The \textit{Track Initialization Module} determines whether to initialize a new track for each unmatched detection.}
    
    \label{fig:arch_deep}
\end{figure*}

